FREESS: An Educational Simulator of a RISC-V-Inspired Superscalar Processor Based on Tomasulo's Algorithm

FREESS is a free, interactive simulator that illustrates instruction-level parallelism in a RISC-V-inspired superscalar processor. Based on an extended version of Tomasulo's algorithm, FREESS is intended as a hands-on educational tool for Advanced Computer Architecture courses. It enables students to explore dynamic, out-of-order instruction execution, emphasizing how instructions are issued as soon as their operands become available. The simulator models key microarchitectural components, including the Instruction Window (IW), Reorder Buffer (ROB), Register Map (RM), Free Pool (FP), and Load/Store Queues. FREESS allows users to dynamically configure runtime parameters, such as the superscalar issue width, functional unit types and latencies, and the sizes of architectural buffers and queues. To simplify learning, the simulator uses a minimal instruction set inspired by RISC-V (ADD, ADDI, BEQ, BNE, LW, MUL, SW), which is sufficient to demonstrate key pipeline stages: fetch, register renaming, out-of-order dispatch, execution, completion, commit, speculative branching, and memory access. FREESS includes three step-by-step, illustrated examples that visually demonstrate how multiple instructions can be issued and executed in parallel within a single cycle. Being open source, FREESS encourages students and educators to experiment freely by writing and analyzing their own instruction-level programs and superscalar architectures.

==> Makefile <==
FIGDIR=FIG

PAPER=$(shell bash -c 'basename `pwd`|cut -d. -f1')
PAPER=2505-WCAE

.PHONY: dvi all figs clean spellcheck veryclean

all: figs $(PAPER).pdf

#	bibtex main
#	biblatex main
$(PAPER).pdf: PAPERTAG.txt main.tex PAPERCUSTOM.tex *.bib *.tex FIG/$(PAPER)*_FIG_*.pdf  FIG/$(PAPER)*_Slide_*.txt
	pdflatex main
#	./puliscibib.sh
	bibtex main
	pdflatex main
	pdflatex main
	@if [ -s main.pdf ]; \
	   rm -f $(PAPER).pdf; \
	   then mv main.pdf $(PAPER).pdf; \
	   echo "* Generated $(PAPER).pdf"; \
	fi

PAPERTAG.txt:
	@rm -f PAPERTAG.txt 2>/dev/null
	echo "$(PAPER)" >PAPERTAG.txt

main.tex:
	@if [ ! -s main.tex ]; then echo "ERROR: cannot find main.tex"; exit 1; fi

PAPERCUSTOM.tex:
	@if [ ! -s main.tex ]; then echo "ERROR: cannot find PAPERCUSTOM.tex"; exit 1; fi

$(FIGDIR)/$(PAPER)-figs.pptm:
	@if [ ! -s $(FIGDIR)/$(PAPER)-figs.pptm ]; then echo "ERROR: cannot find $(FIGDIR)/$(PAPER)-figs.pptm"; exit 1; fi

$(FIGDIR)/$(PAPER)*_FIG_*.pdf: $(FIGDIR)/$(PAPER)-figs.pptm $(FIGDIR)/$(PAPER)*_Slide_*.pdf
	@b=`ls FIG/$(PAPER)*_Slide_*.pdf 2>/dev/null|sed 's/.*Slide_\([0-9]\+\).*/\1/g'|tr -s ' '|sort -n|uniq|tail -1 |tr -d '\n\r'`; \
	if [ -z "$$b" ]; then echo "ERROR: you must produce the Slide*pdf files from the PPTM"; exit 1; fi; \
	cd $(FIGDIR); \
	for i in $(PAPER)*_Slide_*.pdf; do ff=`echo "$$i"|sed 's/_Slide_/_FIG_/'`; rm -f $${i}.tmp $${ff} 2>/dev/null; done; \
	for i in $(PAPER)*_Slide_*.pdf; do cp $${i} $${i}.tmp; done; \
	for i in $(PAPER)*_Slide_*.pdf; do ff=`echo "$$i"|sed 's/_Slide_/_FIG_/'`; nn=`echo "$$i"|sed 's/.*Slide_\([0-9]\+\).pdf/\1/'`; echo "Processing figure $${nn} ..."; /usr/bin/pdfcrop $${i}.tmp $${ff} >/dev/null 2>/dev/null; done; \
	for i in $(PAPER)*_Slide_*.pdf; do rm -f $${i}.tmp 2>/dev/null; done; \
	sleep 1

$(FIGDIR)/$(PAPER)*_FIG_*.eps: pdffigs
	@cd $(FIGDIR); for i in $(PAPER)*_FIG_*.pdf; do /usr/bin/pdftops -f 1 -l 1 -eps $$i; done; \
	ls -l *_FIG_*.eps; sleep 1

$(FIGDIR)/$(PAPER)*_FIG_*.jpg: pdffigs
	@cd $(FIGDIR); for i in $(PAPER)*_FIG_*.pdf; do fig=`echo "$$i" | sed 's/\(.*\)FIG_\([0-9]\+\).pdf/\1FIG_\2/'`; /usr/bin/pdftoppm -r 300 -jpeg -singlefile $$i $$fig; done; \
	ls -l *_FIG_*.jpg; sleep 1

pdffigs: $(FIGDIR)/$(PAPER)*_FIG_*.pdf # $(FIGDIR)/$(PAPER)*_FIG_*.pdf

epsfigs: $(FIGDIR)/$(PAPER)*_FIG_*.pdf # $(FIGDIR)/$(PAPER)*_FIG_*.jpg

jpgfigs: $(FIGDIR)/$(PAPER)*_FIG_*.pdf # $(FIGDIR)/$(PAPER)*_FIG_*.jpg 


dvi: main.dvi

#	bibtex main
#	biblatex main
main.dvi: main.tex *.bib *.tex FIG/$(PAPER)*_FIG_*.pdf  FIG/$(PAPER)*_FIG_*.txt
	latex main
	bibtex main
	latex main
	latex main

gitpull:
	git pull

figs: $(FIGDIR)/$(PAPER)-figs.pptm pdffigs jpgfigs

gitfigs: gitpull figs
	@if [ $$(git status --porcelain FIG | wc -l) -gt 0 ]; then \
            git add FIG && \
            git commit -m "updating FIG" && \
            git push; \
        else \
            echo "Nothing to commit in the FIG directory."; \
        fi

clean:
	rm -rf *.out *.aux *.log *.bbl *.blg *.dvi  *.ps *~ *.pdf $(FIGDIR)/*_FIG_*.eps $(FIGDIR)/*_FIG_*.pdf $(FIGDIR)/*.jpg  $(FIGDIR)/*_Slide_*.pdf.tmp

spellcheck:
	for i in *.tex; do aspell --personal=./personal.wl -c $$i; done

# also removes pdfs
veryclean:
	rm -rf *.out *.aux *.log *.bbl *.blg *.dvi *.pdf *.ps *~ $(FIGDIR)/*eps $(FIGDIR)/*pdf $(FIGDIR)/*txt

